Empowering Vector Architectures for ML: The CAMP Architecture for Matrix Multiplication

This study presents the Cartesian Accumulative Matrix Pipeline (CAMP) architecture, a novel approach designed to enhance matrix multiplication in Vector Architectures (VAs) and Single Instruction Multiple Data (SIMD) units. CAMP improves the processing efficiency of Quantized Neural Networks (QNNs). Matrix multiplication is a cornerstone of machine learning applications, and its quantized versions are increasingly popular for more efficient operations. Unfortunately, existing VAs and SIMD-support units struggle to efficiently handle these quantized formats. In this work, we propose CAMP, a simple yet effective architecture that leverages a hybrid multiplier. The CAMP architecture significantly advances the performance of vector architectures in handling quantized data, enabling more efficient execution of matrix multiplication across various platforms, specifically targeting the ARMv8 Scalable Vector Extension (SVE) and edge RISC-V SIMD-based architectures. In addition to increasing throughput, CAMP's architectural design also contributes to energy efficiency, making it an effective solution for low-power applications. Evaluations on a range of Large Language Models (LLMs) and Convolutional Neural Networks (CNNs) demonstrate that matrix multiplication operations using the proposed micro-architecture achieve up to 17$\times$ and 23$\times$ performance improvements compared to their respective baselines, the ARM A64FX core and a RISC-V-based edge System-on-Chip (SoC). Furthermore, synthesis and place-and-route (PnR) of the CAMP micro-architecture using Synopsys tools -- targeting ARM TSMC 7nm for A64FX and GlobalFoundries 22nm for the RISC-V SoC -- add only 1\% and 4\% area overhead, respectively, compared to the baseline designs.

==> 06_design_space.tex <==
\section{Design Space Exploration} \label{sec:Design_space}

\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{figures/design_space_compress2.pdf}

  \caption{Register array configurations for executing an $8\times8$ matrix multiplication across different clock cycles, demonstrating efficiency optimizations: (a) 64 clocks, (b) 32 clocks, (c) 16 clocks, (d) 8 clocks, (e) 4 clocks. Each configuration illustrates the registers adaptation required to reduce execution time.}
  \label{fig:design_space}

\end{figure*}

As described in Section~\ref{subsec:Microarchitecture}, the number of registers in CAMP micro-architecture, and correspondingly, the number of accumulator units, depends on the number of clock cycles.
This dependency introduces a trade-off between area efficiency and the required latency.
The $camp$ instruction performs matrix multiplication for square matrices, where the input matrices contain sixty-four 8-bit integers, and the outputs are sixty-four 32-bit integers.
Accordingly, the auxiliary register, designed to hold the intermediate results, requires a size of 64$\times$32-bits.
Bearing in mind that the studied architecture's vector length is 512 bits, the final accumulated result will be transferred to a total of four vector registers, as they represent the output of the instruction. The output is sequentially transferred from the $camp$ multiplier to the output registers, one register at a time, across all evaluated configurations.
%once 512 bits of output which is a quarter of auxiliary register are ready, they will be transferred to the output register.

Figure~\ref{fig:design_space}.(a) illustrates the first design of the register array, which requires 64 clock cycles to complete the operation. This design features a single accumulator, and its pipeline architecture allows for the accumulation of results from 8 lanes. The first quarter of the accumulated results (16x32-bit values) is transferred to the output's first vector register after 16 clock cycles.
Thus, after 64 clock cycles, all the required results are stored in the auxiliary register.
Similarly, the second design, Figure~\ref{fig:design_space}.(b), features two accumulators in the inter-lane accumulators.
This design requires 8 clock cycles to generate the first output register and 32 clock cycles to process all the outputs.
Further configurations (Figure~\ref{fig:design_space}.c-e) are equipped with additional accumulators to reduce the number of clock cycles required for calculations. The last configuration generates one output register per cycle and requires only four cycles to fill all the output registers.
To quantify the impact in the area of each configuration, we  implemented all the CAMP configurations using Verilog and synthesized them using the $7\mathrm{nm}$ technology node, which is the same technology used by the ARM A64FX, with a target frequency of 2GHz.
We compare the area overhead of all the evaluated CAMP configurations to an A64FX core using the methodology proposed by \emph{et al.}~\cite{arima2021power}.
Table~\ref{table:clock_area_relative_simulation} reports the area and area overhead results among all the evaluated configurations.
The SoC layouts for various configurations and their relative areas, compared to the A64FX CPU and its core, are depicted in Figure~\ref{fig:layout}. The CAMP layouts shown use a square floorplan, aiming to maximize cell density (around 85\% for all designs) without causing congestion issues.

The design requiring fewer clock cycles occupies a larger area due to the increased number of accumulators and registers needed to store results, aligning with our expectations.
However, compared to the A64FX core, CAMP features a negligible area overhead of 1\% for the larger configurations evaluated.

We assess the performance impact of each CAMP configuration using a general SMM operation, employing matrix sizes from the SMM column in Table~\ref{tab:transposed_benchmark_sizes} and randomly generated values. The performance of the CAMP configurations is compared to all the approaches listed in Section~\ref{sec:experiments}. The results, normalized to the OpenBLAS implementation, are shown in Figure~\ref{fig:exp_gemm}.
%The simulation results are normalized based on the openBLAS approach. Fig.~\ref{fig:exp_gemm} illustrates the speedup of different approaches relative to matrix sizes. 
According to these results, the CAMP architecture significantly outperforms other methods.
We make three observations:
(1)
%Beyond the CAMP$\_$64clk configuration, other CAMP designs demonstrate a substantial advantage over competing approaches, an advantage that becomes more pronounced with increasing matrix sizes.
The 4clk, 8clk, and 16clk configurations significantly outperform aggressive state-of-the-art optimizations, such as OpenBlas.
%whereas the CAMP$\_$32clk shows marginally better performance compared to Gemmlowp methods.
%Given that the 64 clock version's performance is comparable to Gemmlowp, and the 32 clock version is slightly better than Gemmlowp, results for these method are excluded from further benchmarks.
(2) The 32clk and 64clk configurations feature small performance benefits compared to openBLAS and gemmlowp.
For this reason, results reported in Section~\ref{Sec:PERFORMANCE_EVALUATION} only report the performance for the 4clk, 8clk, and 16clk configurations.
(3) CAMP incurs a negligible area overhead while providing significant performance results compared to highly optimized vectorized implementations.
%Furthermore, the performance evaluation of the various configurations is based on the requisite number of clock cycles required to execute square matrix multiplication on a dataset of size $1024$ with randomized entries. The comparison of clock cycles takes into account the slowest design, which requires 64 clock cycles, and the speedup of different designs relative to this design is reported in the last column of the table.

\begin{table}[ht]
\caption{Comparative Analysis of the Area and Performance Metrics of Proposed Configurations Relative to the ARM-Fugaku Core.}
\label{table:clock_area_relative_simulation}
\centering
\begin{tabular}{c c c c}
\hline
\textbf{Design Approach} & \multicolumn{1}{c}{\textbf{Area}} & \multicolumn{1}{c}{\textbf{Relative Area}} & \multicolumn{1}{c}{\textbf{Speedup}} \\
 & \multicolumn{1}{c}{\textit{($m m^2$)}} & \multicolumn{1}{c}{\textit{(\%)}} & \multicolumn{1}{c}{} \\
\hline \\ [-1.5ex]
\textbf{64clk} & 0.0083 & 0.28\% & 1 \\ 
\textbf{32clk} & 0.0094 & 0.32\% & 1.8 \\
\textbf{16clk} & 0.0205 & 0.70\% & 3.1 \\
\textbf{8clk} & 0.0292 & 1.01\% & 4.5 \\
\textbf{4clk} & 0.0304 & 1.04\% & 5.8 \\
\hline
\end{tabular}

\end{table}




\begin{figure}
    \centering
    %\includegraphics[width=\linewidth,trim=50 25 20 15,clip]{figures/hybrid_mult_integration} % <left bottom right top>
    \includegraphics[width=\linewidth]{figures/speedup1.pdf}

    \caption{Comparative speedup across matrix sizes.}
    \label{fig:exp_gemm}

\end{figure}





\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/layout.pdf}

    \caption{Area Comparison between Arm A64FX and Various Configurations of the CAMP Microarchitecture: (a) Die photo of the A64FX CPU, showcasing the overall architecture. (b) Area comparison of the CAMP microarchitecture and a single core from the A64FX, presented at the same scale for direct comparison. (c) Detailed layout for different CAMP design. Lx represents the lane number.}
    \label{fig:layout}

\end{figure*}
